Prospects for measuring supermassive black hole masses with future extremely large telescopes

The next generation of giant-segmented mirror telescopes ($>$ 20 m) will enable us to observe galactic nuclei at much higher angular resolution and sensitivity than ever before. These capabilities will introduce a revolutionary shift in our understanding of the origin and evolution of supermassive black holes by enabling more precise black hole mass measurements in a mass range that is unreachable today. We present simulations and predictions of the observations of nuclei that will be made with the Thirty Meter Telescope (TMT) and the adaptive optics assisted integral-field spectrograph IRIS, which is capable of diffraction-limited spectroscopy from $Z$ band (0.9 $\mu$m) to $K$ band (2.2 $\mu$m). These simulations, for the first time, use realistic values for the sky, telescope, adaptive optics system, and instrument, to determine the expected signal-to-noise ratio of a range of possible targets spanning intermediate mass black holes of $\sim10^4$ \msun to the most massive black holes known today of $>10^{10}$ $M_\odot$. We find that IRIS will be able to observe Milky Way-mass black holes out the distance of the Virgo cluster, and will allow us to observe many more brightest cluster galaxies where the most massive black holes are thought to reside. We also evaluate how well the kinematic moments of the velocity distributions can be constrained at the different spectral resolutions and plate scales designed for IRIS. We find that a spectral resolution of $\sim8000$ will be necessary to measure the masses of intermediate mass black holes. By simulating the observations of galaxies found in SDSS DR7, we find that over $10^5$ massive black holes will be observable at distances between $0.005 < z < 0.18$ with the estimated sensitivity and angular resolution provided by access to $Z$-band (0.9 $\mu$m) spectroscopy from IRIS and the TMT adaptive optics system. (Abridged)

==> lauer_galaxy_sample_table_full.tex <==
NGC 3115  &	 S0-  &	-21.1 &	11.5 &	10.2 &	0.89 &	0.52 &	89. &	394. &	196. &	392. &	1.9e+08 &	18.1 \\
NGC 3607  &	 S0  &	-19.9 &	13.9 &	10.9 &	0.95 &	0.26 &	21. &	96. &	52. &	103. &	5.5e+07 &	9.0 \\
NGC 3384  &	 S0-  &	-19.9 &	13.4 &	11.7 &	1.02 &	0.71 &	85. &	373. &	186. &	372. &	5.8e+07 &	8.6 \\
NGC 3377  &	 E  &	-20.1 &	11.1 &	11.7 &	1.02 &	0.03 &	115. &	506. &	251. &	502. &	6.7e+07 &	9.3 \\
NGC 3379  &	 E  &	-21.1 &	13.2 &	11.7 &	1.02 &	0.18 &	26. &	118. &	62. &	123. &	2.0e+08 &	16.0 \\
NGC 1023  &	 S0-  &	-20.5 &	12.7 &	12.1 &	1.06 &	0.74 &	92. &	399. &	199. &	398. &	1.1e+08 &	11.3 \\
NGC 3056  &	 S0+  &	-19.0 &	15.1 &	12.9 &	1.13 &	0.90 &	90. &	388. &	194. &	388. &	2.2e+07 &	4.8 \\
NGC 4697  &	 E  &	-21.5 &	13.3 &	13.3 &	1.16 &	0.22 &	40. &	177. &	90. &	180. &	2.9e+08 &	16.8 \\
NGC 2549  &	 S0  &	-19.2 &	14.6 &	13.4 &	1.17 &	0.67 &	57. &	247. &	124. &	249. &	2.7e+07 &	5.1 \\
NGC 7457  &	 S0-  &	-18.6 &	13.3 &	14.0 &	1.22 &	-0.10 &	12. &	53. &	32. &	63. &	1.5e+07 &	3.7 \\
NGC 2685  &	 S0+  &	-19.7 &	14.0 &	14.3 &	1.25 &	0.73 &	71. &	310. &	155. &	310. &	4.7e+07 &	6.3 \\
NGC 4150  &	 S0  &	-18.7 &	11.1 &	14.5 &	1.27 &	0.82 &	91. &	394. &	196. &	393. &	1.6e+07 &	3.6 \\
NGC 2841  &	 Sb  &	-20.6 &	11.5 &	15.1 &	1.32 &	0.05 &	33. &	152. &	78. &	156. &	1.1e+08 &	9.3 \\
NGC 4143  &	 S0  &	-19.7 &	14.1 &	15.6 &	1.36 &	0.59 &	66. &	292. &	146. &	292. &	4.5e+07 &	5.7 \\
NGC 4026  &	 S0  &	-19.8 &	12.2 &	15.6 &	1.36 &	0.15 &	74. &	331. &	165. &	330. &	5.0e+07 &	6.0 \\
NGC 2950  &	 S0  &	-19.7 &	13.8 &	15.8 &	1.38 &	0.82 &	102. &	443. &	221. &	441. &	4.7e+07 &	5.8 \\
NGC 4742  &	 E  &	-19.9 &	13.9 &	16.4 &	1.43 &	1.04 &	143. &	610. &	304. &	608. &	5.6e+07 &	6.1 \\
NGC 4278  &	 E  &	-21.1 &	13.2 &	16.7 &	1.46 &	0.06 &	18. &	83. &	46. &	91. &	1.8e+08 &	10.7 \\
NGC 6340  &	 S0  &	-19.5 &	12.4 &	16.8 &	1.47 &	0.59 &	51. &	223. &	113. &	225. &	3.6e+07 &	4.7 \\
NGC 4239  &	 E  &	-18.5 &	14.4 &	17.5 &	1.53 &	-0.06 &	12. &	53. &	32. &	63. &	1.3e+07 &	2.8 \\
NGC 4486  &	 E  &	-22.7 &	14.3 &	17.9 &	1.56 &	0.27 &	15. &	68. &	38. &	77. &	1.0e+09 &	23.3 \\
VCC 1627  &	 E  &	-16.4 &	14.9 &	17.9 &	1.56 &	-0.10 &	18. &	79. &	44. &	87. &	1.6e+06 &	0.9 \\
VCC 1545  &	 E  &	-17.5 &	17.4 &	17.9 &	1.56 &	0.05 &	5. &	23. &	16. &	33. &	4.8e+06 &	1.6 \\
VCC 1440  &	 E  &	-17.2 &	13.9 &	17.9 &	1.56 &	0.14 &	25. &	106. &	57. &	113. &	3.7e+06 &	1.4 \\
VCC 1199  &	 E  &	-15.6 &	16.7 &	17.9 &	1.56 &	-0.08 &	25. &	108. &	57. &	115. &	6.8e+05 &	0.6 \\
NGC 4660  &	 E  &	-20.1 &	13.3 &	17.9 &	1.56 &	0.91 &	124. &	535. &	267. &	533. &	7.1e+07 &	6.2 \\
NGC 4649  &	 E  &	-22.5 &	14.3 &	17.9 &	1.56 &	0.16 &	14. &	63. &	36. &	72. &	8.1e+08 &	21.1 \\
NGC 4636  &	 E  &	-21.9 &	14.1 &	17.9 &	1.56 &	0.16 &	13. &	60. &	35. &	70. &	4.2e+08 &	15.1 \\
NGC 4621  &	 E  &	-21.7 &	12.8 &	17.9 &	1.56 &	0.75 &	124. &	537. &	267. &	535. &	3.7e+08 &	14.2 \\
NGC 4564  &	 E  &	-20.3 &	13.5 &	17.9 &	1.56 &	0.80 &	82. &	355. &	178. &	355. &	8.1e+07 &	6.7 \\
NGC 4552  &	 E  &	-21.6 &	12.2 &	17.9 &	1.56 &	-0.10 &	21. &	88. &	52. &	95. &	3.4e+08 &	13.6 \\
NGC 4551  &	 E  &	-19.4 &	13.5 &	17.9 &	1.56 &	-0.07 &	32. &	139. &	72. &	144. &	3.3e+07 &	4.2 \\
NGC 4503  &	 S0-  &	-19.6 &	14.1 &	17.9 &	1.56 &	0.64 &	45. &	195. &	99. &	198. &	4.0e+07 &	4.7 \\
NGC 4494  &	 E  &	-21.5 &	14.2 &	17.9 &	1.56 &	0.52 &	64. &	284. &	142. &	284. &	2.9e+08 &	12.6 \\
NGC 4374  &	 E  &	-22.3 &	13.0 &	17.9 &	1.56 &	0.15 &	24. &	107. &	57. &	113. &	6.4e+08 &	18.7 \\
NGC 4382  &	 S0+  &	-22.0 &	12.7 &	17.9 &	1.56 &	0.00 &	23. &	104. &	55. &	110. &	4.6e+08 &	15.9 \\
NGC 4387  &	 E  &	-19.2 &	13.8 &	17.9 &	1.56 &	0.10 &	27. &	120. &	63. &	126. &	2.9e+07 &	4.0 \\
NGC 4406  &	 E  &	-22.5 &	13.0 &	17.9 &	1.56 &	-0.04 &	12. &	52. &	32. &	61. &	7.7e+08 &	20.5 \\
NGC 4417  &	 S0  &	-18.9 &	14.6 &	17.9 &	1.56 &	0.71 &	78. &	342. &	171. &	341. &	2.1e+07 &	3.4 \\
NGC 4434  &	 E  &	-19.2 &	13.6 &	17.9 &	1.56 &	-0.04 &	34. &	154. &	79. &	158. &	2.7e+07 &	3.9 \\
NGC 4458  &	 E  &	-19.3 &	10.7 &	17.9 &	1.56 &	0.16 &	49. &	223. &	112. &	224. &	3.0e+07 &	4.0 \\
NGC 4464  &	 E  &	-18.8 &	13.2 &	17.9 &	1.56 &	0.14 &	46. &	206. &	104. &	208. &	1.9e+07 &	3.2 \\
NGC 4467  &	 E  &	-17.5 &	19.9 &	17.9 &	1.56 &	0.94 &	38. &	162. &	84. &	167. &	4.9e+06 &	1.6 \\
NGC 4472  &	 E  &	-22.9 &	13.6 &	17.9 &	1.56 &	0.01 &	10. &	47. &	29. &	57. &	1.2e+09 &	26.1 \\
NGC 4473  &	 E  &	-21.2 &	14.2 &	17.9 &	1.56 &	-0.07 &	23. &	105. &	56. &	111. &	2.0e+08 &	10.6 \\
NGC 4478  &	 E  &	-19.9 &	12.5 &	17.9 &	1.56 &	-0.10 &	17. &	75. &	44. &	83. &	5.6e+07 &	5.5 \\
NGC 4482  &	 E  &	-18.9 &	17.2 &	17.9 &	1.56 &	0.49 &	5. &	23. &	16. &	33. &	2.0e+07 &	3.3 \\
NGC 4486B  &	 cE  &	-18.0 &	11.5 &	17.9 &	1.56 &	-0.10 &	29. &	123. &	68. &	129. &	7.9e+06 &	2.1 \\
NGC 3945  &	 S0+  &	-20.2 &	15.6 &	19.9 &	1.74 &	-0.06 &	37. &	166. &	85. &	169. &	8.0e+07 &	6.0 \\
NGC 1052  &	 E  &	-21.2 &	11.6 &	20.5 &	1.79 &	0.18 &	42. &	189. &	96. &	192. &	2.1e+08 &	9.3 \\
NGC 1374  &	 E  &	-20.6 &	11.6 &	20.9 &	1.82 &	-0.09 &	28. &	127. &	67. &	132. &	1.1e+08 &	6.7 \\
NGC 1427  &	 E  &	-20.8 &	13.2 &	21.0 &	1.83 &	0.30 &	40. &	178. &	91. &	181. &	1.4e+08 &	7.4 \\
NGC 1553  &	 S0  &	-22.1 &	13.9 &	21.0 &	1.83 &	0.74 &	96. &	420. &	209. &	418. &	5.1e+08 &	14.3 \\
NGC 1351  &	 S0-  &	-20.1 &	13.3 &	21.0 &	1.83 &	0.78 &	74. &	322. &	161. &	322. &	6.8e+07 &	5.2 \\
NGC 1399  &	 E  &	-22.1 &	14.2 &	21.1 &	1.84 &	0.09 &	11. &	51. &	30. &	61. &	5.2e+08 &	14.3 \\
NGC 3585  &	 E  &	-21.9 &	11.7 &	21.2 &	1.85 &	0.31 &	48. &	217. &	109. &	219. &	4.5e+08 &	13.2 \\
NGC 4474  &	 S0  &	-18.4 &	15.6 &	21.6 &	1.88 &	0.72 &	41. &	178. &	91. &	182. &	1.2e+07 &	2.2 \\
NGC 4365  &	 E  &	-22.2 &	13.9 &	21.6 &	1.88 &	0.07 &	12. &	55. &	32. &	64. &	5.8e+08 &	14.7 \\
NGC 7727  &	 Sa  &	-21.2 &	15.4 &	21.6 &	1.88 &	0.43 &	40. &	176. &	90. &	179. &	2.1e+08 &	8.9 \\
NGC 7743  &	 S0+  &	-20.2 &	11.4 &	21.9 &	1.91 &	0.50 &	57. &	251. &	126. &	252. &	7.5e+07 &	5.2 \\
NGC 0584  &	 E  &	-21.4 &	12.2 &	22.1 &	1.93 &	-0.01 &	46. &	208. &	105. &	209. &	2.6e+08 &	9.6 \\
NGC 0596  &	 E  &	-20.9 &	12.9 &	22.1 &	1.93 &	0.16 &	44. &	195. &	99. &	198. &	1.6e+08 &	7.5 \\
NGC 5838  &	 S0-  &	-20.5 &	14.7 &	22.2 &	1.94 &	0.93 &	117. &	504. &	251. &	502. &	1.0e+08 &	6.1 \\
NGC 3610  &	 E  &	-21.0 &	13.4 &	22.6 &	1.97 &	0.76 &	96. &	416. &	207. &	414. &	1.7e+08 &	7.6 \\
NGC 1316  &	 E  &	-23.3 &	11.4 &	22.7 &	1.98 &	-0.10 &	37. &	166. &	86. &	169. &	1.9e+09 &	25.1 \\
NGC 1172  &	 E  &	-20.1 &	13.7 &	22.7 &	1.98 &	-0.01 &	48. &	212. &	107. &	214. &	7.1e+07 &	4.9 \\
NGC 7213  &	 Sa  &	-21.7 &	14.7 &	22.7 &	1.98 &	0.06 &	18. &	84. &	46. &	91. &	3.6e+08 &	11.0 \\
NGC 2974  &	 E  &	-21.1 &	12.4 &	22.7 &	1.98 &	0.62 &	56. &	246. &	124. &	248. &	1.9e+08 &	8.0 \\
NGC 2434  &	 E  &	-21.3 &	16.1 &	22.8 &	1.99 &	0.75 &	41. &	179. &	91. &	183. &	2.4e+08 &	9.0 \\
NGC 3608  &	 E  &	-21.1 &	12.7 &	23.0 &	2.01 &	0.09 &	29. &	129. &	67. &	134. &	2.0e+08 &	8.1 \\
NGC 3599  &	 S0  &	-19.9 &	14.4 &	23.0 &	2.01 &	0.75 &	41. &	176. &	90. &	180. &	5.8e+07 &	4.4 \\
NGC 3605  &	 E  &	-19.6 &	14.2 &	23.0 &	2.01 &	0.59 &	31. &	134. &	70. &	140. &	4.2e+07 &	3.7 \\
NGC 1331  &	 E  &	-18.6 &	16.3 &	24.2 &	2.11 &	0.57 &	13. &	55. &	32. &	65. &	1.5e+07 &	2.1 \\
NGC 2778  &	 E  &	-18.8 &	13.1 &	24.2 &	2.11 &	0.33 &	52. &	230. &	116. &	231. &	1.7e+07 &	2.3 \\
NGC 7332  &	 S0  &	-19.6 &	12.9 &	24.3 &	2.12 &	0.62 &	94. &	412. &	205. &	410. &	4.2e+07 &	3.5 \\
NGC 4589  &	 E  &	-21.4 &	13.1 &	25.0 &	2.18 &	0.21 &	26. &	119. &	62. &	125. &	2.5e+08 &	8.3 \\
NGC 4291  &	 E  &	-20.6 &	12.7 &	25.0 &	2.18 &	0.01 &	22. &	99. &	53. &	106. &	1.2e+08 &	5.8 \\
NGC 4121  &	 E  &	-18.5 &	17.3 &	25.2 &	2.20 &	0.85 &	50. &	217. &	110. &	220. &	1.4e+07 &	2.0 \\
NGC 0524  &	 S0+  &	-21.9 &	13.1 &	25.4 &	2.22 &	0.25 &	32. &	145. &	75. &	149. &	4.1e+08 &	10.6 \\
NGC 0821  &	 E  &	-21.7 &	12.7 &	25.5 &	2.23 &	0.10 &	48. &	214. &	108. &	216. &	3.6e+08 &	9.8 \\
NGC 1439  &	 E  &	-20.8 &	13.2 &	26.5 &	2.31 &	0.74 &	59. &	256. &	129. &	257. &	1.4e+08 &	6.0 \\
NGC 1426  &	 E  &	-20.8 &	14.0 &	26.5 &	2.31 &	0.25 &	38. &	168. &	86. &	172. &	1.4e+08 &	5.9 \\
NGC 1400  &	 S0-  &	-21.4 &	12.4 &	26.5 &	2.31 &	-0.10 &	21. &	96. &	52. &	103. &	2.5e+08 &	7.9 \\
NGC 3414  &	 S0  &	-20.2 &	14.1 &	26.7 &	2.33 &	0.83 &	80. &	345. &	173. &	345. &	8.0e+07 &	4.4 \\
NGC 5061  &	 E  &	-22.0 &	11.3 &	26.9 &	2.35 &	0.04 &	41. &	186. &	94. &	188. &	4.9e+08 &	10.9 \\
UGC 4551  &	 S0  &	-19.8 &	14.7 &	27.1 &	2.36 &	0.51 &	30. &	133. &	69. &	138. &	5.0e+07 &	3.4 \\
NGC 5576  &	 E  &	-21.3 &	14.8 &	27.1 &	2.36 &	0.01 &	42. &	187. &	95. &	190. &	2.4e+08 &	7.5 \\
NGC 2592  &	 E  &	-20.0 &	14.2 &	27.2 &	2.37 &	0.92 &	78. &	335. &	168. &	336. &	6.3e+07 &	3.9 \\
NGC 4648  &	 E  &	-20.2 &	13.5 &	27.7 &	2.42 &	0.92 &	95. &	408. &	204. &	407. &	8.0e+07 &	4.3 \\
NGC 3640  &	 E  &	-22.0 &	12.7 &	28.3 &	2.47 &	-0.10 &	23. &	107. &	56. &	113. &	4.6e+08 &	10.1 \\
NGC 2699  &	 E  &	-20.2 &	15.2 &	28.4 &	2.48 &	0.84 &	61. &	263. &	132. &	265. &	8.0e+07 &	4.2 \\
NGC 5812  &	 E  &	-21.4 &	14.2 &	28.4 &	2.48 &	0.59 &	46. &	204. &	103. &	207. &	2.6e+08 &	7.5 \\
NGC 5845  &	 E  &	-20.0 &	12.9 &	28.7 &	2.50 &	0.51 &	65. &	288. &	144. &	288. &	6.1e+07 &	3.6 \\
NGC 5813  &	 E  &	-22.0 &	13.9 &	28.7 &	2.50 &	-0.10 &	12. &	50. &	31. &	60. &	4.9e+08 &	10.2 \\
NGC 5831  &	 E  &	-21.0 &	14.5 &	28.7 &	2.50 &	0.33 &	40. &	177. &	90. &	181. &	1.7e+08 &	6.1 \\
NGC 0720  &	 E  &	-22.2 &	14.4 &	29.2 &	2.55 &	0.06 &	7. &	33. &	22. &	43. &	5.9e+08 &	11.0 \\
NGC 0474  &	 S0  &	-20.1 &	14.2 &	29.3 &	2.56 &	0.37 &	28. &	126. &	66. &	132. &	7.0e+07 &	3.8 \\
NGC 3266  &	 S0  &	-20.1 &	15.4 &	29.4 &	2.57 &	0.64 &	35. &	151. &	78. &	156. &	7.0e+07 &	3.8 \\
NGC 3065  &	 S0  &	-19.6 &	15.6 &	29.6 &	2.58 &	0.79 &	65. &	283. &	142. &	284. &	4.3e+07 &	2.9 \\
NGC 3900  &	 S0+  &	-20.8 &	12.2 &	29.9 &	2.61 &	0.51 &	86. &	370. &	185. &	370. &	1.4e+08 &	5.3 \\
NGC 2300  &	 S0  &	-21.7 &	14.5 &	30.4 &	2.65 &	0.07 &	11. &	48. &	29. &	58. &	3.7e+08 &	8.4 \\
NGC 3613  &	 E  &	-21.6 &	12.7 &	30.8 &	2.69 &	0.04 &	19. &	86. &	47. &	93. &	3.2e+08 &	7.6 \\
IC 1459  &	 E  &	-22.5 &	13.4 &	30.9 &	2.70 &	-0.10 &	21. &	96. &	53. &	103. &	8.1e+08 &	12.2 \\
NGC 5308  &	 S0-  &	-21.3 &	13.2 &	33.0 &	2.88 &	0.82 &	102. &	442. &	220. &	441. &	2.3e+08 &	6.0 \\
NGC 2902  &	 S0  &	-20.6 &	13.9 &	33.0 &	2.88 &	0.49 &	30. &	130. &	68. &	136. &	1.1e+08 &	4.3 \\
NGC 5903  &	 E  &	-21.9 &	14.4 &	33.3 &	2.91 &	0.13 &	10. &	43. &	27. &	53. &	4.4e+08 &	8.3 \\
NGC 5898  &	 E  &	-21.6 &	13.9 &	33.3 &	2.91 &	0.41 &	31. &	136. &	71. &	141. &	3.4e+08 &	7.3 \\
NGC 4261  &	 E  &	-22.3 &	13.4 &	33.4 &	2.91 &	0.16 &	19. &	84. &	46. &	92. &	6.3e+08 &	9.9 \\
NGC 2907  &	 Sa  &	-21.2 &	13.6 &	34.4 &	3.00 &	0.58 &	96. &	420. &	209. &	418. &	2.2e+08 &	5.7 \\
NGC 4128  &	 S0  &	-20.8 &	13.9 &	34.5 &	3.01 &	0.71 &	70. &	306. &	153. &	307. &	1.4e+08 &	4.5 \\
NGC 3595  &	 E  &	-21.0 &	15.0 &	35.2 &	3.07 &	0.75 &	44. &	189. &	96. &	193. &	1.7e+08 &	4.8 \\
NGC 2634  &	 E  &	-20.8 &	14.9 &	35.3 &	3.08 &	0.81 &	48. &	209. &	106. &	212. &	1.5e+08 &	4.5 \\
NGC 3193  &	 E  &	-22.0 &	13.1 &	36.0 &	3.14 &	0.01 &	34. &	155. &	79. &	159. &	4.7e+08 &	8.0 \\
NGC 4709  &	 E  &	-22.3 &	14.5 &	37.0 &	3.23 &	0.27 &	14. &	61. &	35. &	70. &	6.7e+08 &	9.2 \\
NGC 3078  &	 E  &	-21.9 &	14.8 &	37.2 &	3.25 &	0.95 &	102. &	440. &	220. &	439. &	4.6e+08 &	7.6 \\
NGC 4168  &	 E  &	-21.8 &	15.1 &	37.3 &	3.26 &	0.17 &	8. &	35. &	23. &	46. &	3.9e+08 &	7.0 \\
NGC 2986  &	 E  &	-22.3 &	13.7 &	37.6 &	3.28 &	0.18 &	17. &	78. &	43. &	86. &	6.7e+08 &	9.1 \\
IC 1565  &	 BCG  &	-23.0 &	13.9 &	38.2 &	3.33 &	-0.20 &	8. &	31. &	22. &	41. &	1.3e+09 &	12.6 \\
NGC 5198  &	 E  &	-21.2 &	12.4 &	38.3 &	3.34 &	0.23 &	25. &	115. &	60. &	120. &	2.2e+08 &	5.1 \\
NGC 2636  &	 E  &	-19.2 &	13.5 &	38.3 &	3.34 &	0.06 &	23. &	100. &	54. &	107. &	2.7e+07 &	1.8 \\
NGC 6278  &	 S0  &	-20.8 &	13.3 &	40.0 &	3.49 &	0.55 &	55. &	243. &	122. &	244. &	1.4e+08 &	4.0 \\
NGC 4696  &	 BCG  &	-24.3 &	14.8 &	40.0 &	3.49 &	0.10 &	5. &	22. &	16. &	32. &	5.2e+09 &	23.9 \\
NGC 5017  &	 E  &	-20.7 &	14.5 &	40.3 &	3.52 &	1.12 &	115. &	489. &	244. &	489. &	1.2e+08 &	3.7 \\
NGC 5982  &	 E  &	-22.0 &	12.7 &	40.5 &	3.53 &	0.05 &	18. &	84. &	46. &	92. &	4.7e+08 &	7.1 \\
NGC 1700  &	 E  &	-21.9 &	10.6 &	40.6 &	3.54 &	-0.10 &	51. &	232. &	116. &	232. &	4.6e+08 &	7.0 \\
NGC 3348  &	 E  &	-22.2 &	13.6 &	41.5 &	3.62 &	0.09 &	17. &	77. &	42. &	85. &	5.8e+08 &	7.7 \\
ESO 447-30  &	 S0  &	-21.2 &	14.3 &	41.7 &	3.64 &	0.84 &	65. &	282. &	142. &	283. &	2.1e+08 &	4.6 \\
IC 0875  &	 S0  &	-20.2 &	15.3 &	41.9 &	3.66 &	1.07 &	104. &	444. &	222. &	445. &	7.7e+07 &	2.8 \\
UGC 6062  &	 S0  &	-20.3 &	16.0 &	42.2 &	3.68 &	0.80 &	46. &	199. &	101. &	203. &	8.8e+07 &	2.9 \\
NGC 5077  &	 E  &	-22.1 &	14.1 &	44.9 &	3.92 &	0.23 &	21. &	93. &	50. &	101. &	5.2e+08 &	6.7 \\
NGC 5796  &	 E  &	-22.0 &	13.8 &	45.2 &	3.94 &	0.41 &	39. &	171. &	87. &	174. &	4.7e+08 &	6.4 \\
NGC 5370  &	 S0  &	-20.6 &	15.4 &	45.2 &	3.94 &	0.62 &	29. &	125. &	65. &	131. &	1.2e+08 &	3.1 \\
UGC 4587  &	 S0  &	-20.8 &	13.1 &	45.9 &	4.01 &	0.72 &	42. &	182. &	93. &	185. &	1.4e+08 &	3.4 \\
NGC 3706  &	 S0-  &	-22.3 &	11.2 &	46.9 &	4.09 &	-0.01 &	31. &	142. &	74. &	146. &	6.6e+08 &	7.3 \\
ESO 443-39  &	 S0  &	-20.9 &	14.9 &	47.2 &	4.12 &	0.75 &	38. &	163. &	84. &	168. &	1.6e+08 &	3.6 \\
NGC 2872  &	 E  &	-21.6 &	15.7 &	47.4 &	4.14 &	1.01 &	89. &	378. &	190. &	379. &	3.3e+08 &	5.0 \\
ESO 378-20  &	 S0  &	-21.0 &	15.2 &	47.7 &	4.16 &	0.86 &	113. &	483. &	241. &	482. &	1.7e+08 &	3.6 \\
MCG 8-27-18  &	 S0  &	-20.0 &	16.2 &	48.7 &	4.25 &	0.79 &	38. &	163. &	84. &	168. &	6.4e+07 &	2.2 \\
MCG 11-14-25A  &	 E  &	-19.1 &	14.2 &	49.0 &	4.28 &	0.00 &	18. &	81. &	45. &	89. &	2.4e+07 &	1.3 \\
NGC 7785  &	 E  &	-22.1 &	12.1 &	49.9 &	4.35 &	-0.10 &	22. &	102. &	54. &	109. &	5.2e+08 &	6.1 \\
ESO 507-27  &	 S0  &	-20.9 &	15.6 &	50.1 &	4.37 &	0.70 &	53. &	230. &	116. &	232. &	1.6e+08 &	3.3 \\
NGC 5557  &	 E  &	-22.6 &	13.4 &	52.7 &	4.60 &	0.02 &	21. &	97. &	52. &	104. &	9.1e+08 &	7.6 \\
NGC 7626  &	 E  &	-22.9 &	12.7 &	56.0 &	4.89 &	0.47 &	41. &	179. &	91. &	183. &	1.2e+09 &	8.1 \\
NGC 7619  &	 E  &	-22.9 &	13.4 &	56.1 &	4.90 &	-0.02 &	16. &	73. &	41. &	81. &	1.3e+09 &	8.4 \\
IC 4329  &	 BCG  &	-23.9 &	13.4 &	56.7 &	4.95 &	0.01 &	11. &	51. &	30. &	61. &	3.5e+09 &	13.9 \\
NGC 1600  &	 E  &	-23.0 &	16.0 &	57.4 &	5.01 &	-0.03 &	3. &	14. &	12. &	23. &	1.4e+09 &	8.5 \\
NGC 6876  &	 E  &	-23.6 &	14.0 &	57.6 &	5.03 &	0.00 &	6. &	26. &	18. &	36. &	2.4e+09 &	11.3 \\
NGC 5419  &	 E  &	-23.4 &	14.9 &	62.6 &	5.46 &	-0.10 &	5. &	18. &	16. &	27. &	2.0e+09 &	9.3 \\
NGC 0507  &	 S0  &	-23.0 &	14.2 &	63.8 &	5.57 &	0.00 &	10. &	46. &	28. &	56. &	1.4e+09 &	7.7 \\
NGC 7052  &	 E  &	-22.4 &	13.3 &	67.1 &	5.86 &	0.16 &	16. &	73. &	41. &	82. &	6.9e+08 &	5.2 \\
NGC 0741  &	 E  &	-23.3 &	14.7 &	70.9 &	6.19 &	0.10 &	6. &	29. &	19. &	39. &	1.8e+09 &	7.8 \\
NGC 7014  &	 BCG  &	-22.2 &	12.6 &	71.1 &	6.20 &	0.08 &	19. &	87. &	47. &	95. &	5.8e+08 &	4.5 \\
ESO 507-45  &	 S0  &	-23.3 &	12.3 &	73.3 &	6.40 &	0.16 &	30. &	137. &	71. &	142. &	1.8e+09 &	7.6 \\
NGC 0545  &	 BCG  &	-23.0 &	13.9 &	73.3 &	6.40 &	0.08 &	12. &	53. &	32. &	63. &	1.3e+09 &	6.5 \\
NGC 1016  &	 E  &	-22.9 &	15.0 &	75.9 &	6.62 &	0.09 &	10. &	44. &	27. &	54. &	1.2e+09 &	6.1 \\
ESO 462-15  &	 E  &	-22.8 &	13.6 &	80.3 &	7.01 &	-0.10 &	33. &	145. &	75. &	150. &	1.1e+09 &	5.5 \\
NGC 0910  &	 BCG  &	-22.8 &	13.9 &	81.1 &	7.08 &	-0.03 &	6. &	28. &	20. &	38. &	1.1e+09 &	5.4 \\
IC 4931  &	 BCG  &	-23.5 &	14.1 &	83.3 &	7.27 &	0.09 &	9. &	43. &	27. &	53. &	2.2e+09 &	7.4 \\
NGC 6849  &	 S0  &	-22.8 &	14.0 &	84.0 &	7.33 &	0.01 &	10. &	44. &	27. &	54. &	1.1e+09 &	5.2 \\
NGC 4073  &	 E  &	-23.5 &	13.5 &	92.2 &	8.05 &	-0.08 &	8. &	33. &	24. &	44. &	2.2e+09 &	6.8 \\
NGC 4889  &	 BCG  &	-23.7 &	15.0 &	95.0 &	8.29 &	0.03 &	4. &	19. &	14. &	29. &	2.8e+09 &	7.4 \\
NGC 2832  &	 BCG  &	-23.8 &	14.4 &	96.8 &	8.45 &	0.02 &	7. &	32. &	21. &	43. &	2.9e+09 &	7.4 \\
NGC 3842  &	 BCG  &	-23.2 &	14.8 &	97.0 &	8.46 &	0.15 &	8. &	35. &	22. &	45. &	1.6e+09 &	5.5 \\
IC 1633  &	 BCG  &	-23.9 &	14.0 &	98.4 &	8.59 &	-0.02 &	9. &	43. &	27. &	53. &	3.4e+09 &	7.8 \\
NGC 4874  &	 E  &	-23.5 &	16.4 &	106.6 &	9.30 &	0.12 &	2. &	10. &	9. &	18. &	2.2e+09 &	5.8 \\
A0634-M1  &	 BCG  &	-22.7 &	14.1 &	117.3 &	10.24 &	-0.05 &	6. &	24. &	18. &	34. &	9.8e+08 &	3.5 \\
IC 5353  &	 BCG  &	-22.6 &	13.8 &	124.0 &	10.82 &	0.03 &	12. &	55. &	32. &	65. &	9.3e+08 &	3.2 \\
NGC 6173  &	 BCG  &	-23.6 &	14.3 &	126.2 &	11.01 &	-0.33 &	9. &	40. &	26. &	50. &	2.4e+09 &	5.2 \\
A0496-M1  &	 BCG  &	-24.3 &	15.2 &	126.9 &	11.07 &	0.10 &	4. &	17. &	13. &	26. &	5.0e+09 &	7.3 \\
A3747-M1  &	 BCG  &	-22.6 &	13.0 &	128.6 &	11.22 &	-0.02 &	13. &	60. &	35. &	69. &	9.4e+08 &	3.1 \\
A0999-M1  &	 BCG  &	-22.4 &	14.5 &	128.9 &	11.25 &	-0.06 &	7. &	33. &	22. &	44. &	7.6e+08 &	2.8 \\
IC 0613  &	 BCG  &	-22.3 &	13.4 &	128.9 &	11.25 &	0.24 &	15. &	67. &	38. &	76. &	6.3e+08 &	2.6 \\
NGC 3551  &	 BCG  &	-23.6 &	14.6 &	130.1 &	11.35 &	0.13 &	7. &	32. &	21. &	42. &	2.4e+09 &	4.9 \\
NGC 6086  &	 BCG  &	-23.1 &	14.8 &	131.2 &	11.45 &	-0.01 &	6. &	28. &	19. &	38. &	1.5e+09 &	3.9 \\
NGC 1500  &	 BCG  &	-22.8 &	13.7 &	132.5 &	11.56 &	0.08 &	12. &	57. &	33. &	66. &	1.0e+09 &	3.2 \\
A0397-M1  &	 BCG  &	-23.4 &	15.0 &	132.9 &	11.60 &	0.07 &	4. &	20. &	15. &	29. &	2.1e+09 &	4.5 \\
A0189-M1  &	 BCG  &	-21.9 &	14.6 &	133.4 &	11.64 &	0.85 &	10. &	41. &	26. &	52. &	4.3e+08 &	2.1 \\
IC 0664  &	 BCG  &	-22.9 &	12.9 &	138.9 &	12.12 &	0.12 &	15. &	70. &	39. &	78. &	1.2e+09 &	3.2 \\
A2147-M1  &	 BCG  &	-23.2 &	16.5 &	140.0 &	12.22 &	0.18 &	3. &	12. &	10. &	20. &	1.6e+09 &	3.8 \\
IC 0712  &	 BCG  &	-23.3 &	15.1 &	140.7 &	12.28 &	0.17 &	6. &	29. &	20. &	39. &	1.8e+09 &	4.0 \\
A3570-M1  &	 BCG  &	-22.5 &	13.6 &	142.3 &	12.42 &	0.00 &	13. &	58. &	34. &	68. &	8.4e+08 &	2.7 \\
IC 1733  &	 BCG  &	-23.4 &	14.7 &	150.4 &	13.12 &	-0.01 &	4. &	18. &	14. &	27. &	2.1e+09 &	4.0 \\
A0548-M1  &	 BCG  &	-22.8 &	14.5 &	152.6 &	13.32 &	0.00 &	8. &	35. &	23. &	45. &	1.0e+09 &	2.8 \\
IC 2738  &	 BCG  &	-22.2 &	13.6 &	152.7 &	13.33 &	0.53 &	18. &	81. &	44. &	89. &	5.8e+08 &	2.1 \\
A0419-M1  &	 BCG  &	-21.8 &	14.8 &	156.0 &	13.61 &	0.33 &	11. &	48. &	29. &	58. &	3.9e+08 &	1.7 \\
A0295-M1  &	 BCG  &	-23.1 &	14.9 &	168.1 &	14.67 &	0.13 &	5. &	22. &	16. &	31. &	1.5e+09 &	3.0 \\
NGC 7647  &	 BCG  &	-24.0 &	14.2 &	171.4 &	14.96 &	0.04 &	6. &	28. &	19. &	38. &	3.6e+09 &	4.6 \\
IC 0115  &	 BCG  &	-22.7 &	14.5 &	171.7 &	14.98 &	0.09 &	7. &	31. &	21. &	41. &	9.6e+08 &	2.4 \\
NGC 7578B  &	 BCG  &	-23.4 &	13.3 &	171.9 &	15.00 &	0.10 &	14. &	61. &	35. &	70. &	2.0e+09 &	3.5 \\
A3144-M1  &	 BCG  &	-22.3 &	14.2 &	173.0 &	15.10 &	0.07 &	9. &	41. &	25. &	51. &	6.4e+08 &	1.9 \\
A0912-M1  &	 BCG  &	-22.2 &	13.8 &	176.0 &	15.36 &	0.48 &	15. &	66. &	38. &	75. &	6.2e+08 &	1.9 \\
A1983-M1  &	 BCG  &	-22.4 &	12.8 &	176.1 &	15.37 &	-1.37 &	18. &	84. &	46. &	92. &	6.9e+08 &	2.0 \\
A2040-M1  &	 BCG  &	-23.5 &	14.8 &	176.6 &	15.41 &	0.16 &	7. &	30. &	20. &	41. &	2.1e+09 &	3.5 \\
A1631-M1  &	 BCG  &	-23.3 &	13.7 &	176.7 &	15.42 &	-0.03 &	10. &	45. &	28. &	55. &	1.9e+09 &	3.3 \\
A0119-M1  &	 BCG  &	-24.0 &	15.6 &	177.9 &	15.52 &	0.06 &	2. &	11. &	9. &	18. &	3.8e+09 &	4.6 \\
A0168-M1  &	 BCG  &	-23.1 &	13.6 &	177.9 &	15.52 &	-0.48 &	7. &	31. &	22. &	42. &	1.5e+09 &	2.9 \\
A0533-M1  &	 BCG  &	-22.7 &	14.3 &	179.4 &	15.66 &	0.06 &	7. &	33. &	22. &	43. &	9.6e+08 &	2.3 \\
A3716-M1  &	 BCG  &	-23.8 &	15.0 &	180.2 &	15.73 &	-0.03 &	3. &	14. &	11. &	22. &	2.9e+09 &	3.9 \\
A3554-M1  &	 BCG  &	-24.0 &	15.4 &	180.9 &	15.79 &	0.04 &	3. &	11. &	10. &	19. &	3.7e+09 &	4.4 \\
A0261-M1  &	 BCG  &	-22.9 &	15.2 &	181.6 &	15.85 &	0.76 &	6. &	23. &	17. &	33. &	1.3e+09 &	2.6 \\
A3556-M1  &	 BCG  &	-23.6 &	14.2 &	183.0 &	15.97 &	0.09 &	8. &	38. &	24. &	48. &	2.6e+09 &	3.7 \\
A3395-M1  &	 BCG  &	-24.2 &	15.1 &	186.1 &	16.24 &	0.03 &	3. &	14. &	11. &	23. &	4.7e+09 &	4.9 \\
A3564-M1  &	 BCG  &	-22.7 &	14.0 &	186.2 &	16.25 &	0.05 &	10. &	46. &	28. &	56. &	9.6e+08 &	2.2 \\
A3677-M1  &	 BCG  &	-22.2 &	13.9 &	186.6 &	16.28 &	-0.04 &	10. &	46. &	28. &	56. &	6.0e+08 &	1.7 \\
IC 1695  &	 BCG  &	-23.9 &	14.0 &	192.0 &	16.76 &	0.23 &	12. &	54. &	32. &	64. &	3.4e+09 &	4.0 \\
A0376-M1  &	 BCG  &	-23.6 &	15.4 &	195.2 &	17.03 &	0.19 &	5. &	21. &	15. &	30. &	2.5e+09 &	3.4 \\
A3736-M1  &	 BCG  &	-24.0 &	15.3 &	196.2 &	17.12 &	0.11 &	5. &	22. &	16. &	32. &	3.6e+09 &	4.1 \\
A3528-M1  &	 BCG  &	-24.3 &	14.8 &	204.6 &	17.85 &	0.18 &	7. &	30. &	20. &	40. &	5.0e+09 &	4.6 \\
A3532-M1  &	 BCG  &	-24.6 &	14.7 &	208.6 &	18.20 &	0.18 &	7. &	29. &	20. &	40. &	6.7e+09 &	5.2 \\
A1020-M1  &	 BCG  &	-22.6 &	14.1 &	278.6 &	24.31 &	-0.09 &	7. &	31. &	21. &	42. &	9.4e+08 &	1.5 \\
A1831-M1  &	 BCG  &	-23.5 &	15.6 &	321.0 &	28.01 &	0.12 &	2. &	11. &	9. &	18. &	2.2e+09 &	2.0 \\

